Synthesizing Abstract Transformers

This paper addresses the problem of creating abstract transformers automatically. The method we present automates the construction of static analyzers in a fashion similar to the way $\textit{yacc}$ automates the construction of parsers. Our method treats the problem as a program-synthesis problem. The user provides specifications of (i) the concrete semantics of a given operation $\textit{op}$, (ii) the abstract domain A to be used by the analyzer, and (iii) the semantics of a domain-specific language $L$ in which the abstract transformer is to be expressed. As output, our method creates an abstract transformer for $\textit{op}$ in abstract domain A, expressed in $L$ (an "$L$-transformer for $\textit{op}$ over A"). Moreover, the abstract transformer obtained is a most-precise $L$-transformer for $\textit{op}$ over A; that is, there is no other $L$-transformer for $\textit{op}$ over A that is strictly more precise. We implemented our method in a tool called AMURTH. We used AMURTH to create sets of replacement abstract transformers for those used in two existing analyzers, and obtained essentially identical performance. However, when we compared the existing transformers with the transformers obtained using AMURTH, we discovered that four of the existing transformers were unsound, which demonstrates the risk of using manually created transformers.

==> fig/consistent_one.tex <==
\begin{figure}
	\begin{tikzpicture}
		\draw[color=green!60!black,  rotate=20, thick](0,0) ellipse (2.7 and 2);
		\draw[color=red!60, fill=red!5, rotate=-30,  very thick, dashed](0,0) ellipse (2 and 1.8);
		\draw[color=blue!60, fill=blue!5, rotate=30, very thick] (0,0) ellipse (1.5 and 1.75);
		\node[star,star points=4, fill=red, scale=.5, xshift=-4cm, yshift=-1.8cm] (neg1)  {};
%\draw[ultra thick, ->] (6.5,0) arc (0:220:1);
\end{tikzpicture}

\end{figure}

==> fig/negex.tex <==
%pos ex
\begin{tikzpicture}[scale=0.7]
%circle, outermost first
\draw[red, fill=red!0, ] (1.6,-1) ellipse (4.6 and 2.3);
\draw[red, fill=red!0, ] (2,-1) ellipse (4 and 1.8);
\draw[red, fill=red!0, ] (2,-1) ellipse (3 and 1.5);
\draw[red, fill=red!0, ] (2.2,-1) ellipse (2.2 and 1.2);
%\node[star,fill=red,minimum width=1cm] at (0,0) {};

%all the stars
\node[star,fill=red, star points=5, star point ratio=.3] at (-2.5,-1.5) (p3) {$$};
\node[star,fill=red, star points=5, star point ratio=.3] at (5.5,-1) (p2) {$$};
\node[star,fill=red, star points=5, star point ratio=.3] at (-.5,-1) (p1) {$$};
%\node[star,fill=red, star points=5, star point ratio=.3] at (5.35,-0.4) (p4) {$$};


%posex circles
\node[circle,fill=blue] at (1.5,-1) (c1) {$$};
\node[circle,fill=blue] at (2.5,-.5) (c2) {$$};
\node[circle,fill=blue] at (3,-1.5) (c3) {$$};
\end{tikzpicture}

==> fig/posex.tex <==
%pos ex
\begin{tikzpicture}[scale=.6]
%circle, outermost first
\draw[blue, fill=blue!0, ] (2.9,0) ellipse (4.3 and 2);
\draw[brown, fill=blue!0, very thick, dashed] (2.9,0) ellipse (3.2 and 1.65);
\draw[blue, fill=blue!0, ] (2.6,0) ellipse (2.5 and 1.3);
\draw[blue, fill=blue!0, ] (2.3,0) ellipse (1.4 and 0.9);
%\node[star,fill=red,minimum width=1cm] at (0,0) {};

%all the stars
\node[star,fill=blue, star points=5, star point ratio=.3] at (5.35,-0.4) (p3) {$$};
\node[star,fill=blue, star points=5, star point ratio=.3] at (4,0.8) (p2) {$$};
\node[star,fill=blue, star points=5, star point ratio=.3] at (2.8,0) (p1) {$$};
%\node[star,fill=blue, star points=5, star point ratio=.3] at (-.36,0) (p4) {$$};


%naming
\node (name2) [above= of p3, yshift=-1cm, xshift=2mm] {$p3$};
\node (name2) [below= of p2, yshift=1.2cm, xshift=2mm] {$p2$};
\node (name2) [left= of p1, xshift=1cm] {$p3$};
\end{tikzpicture}

==> sections/extra.tex <==

\begin{algorithm2e}
%<<<<<<< HEAD
    \footnotesize
    \DontPrintSemicolon
        $\abst{f}{} \gets \lambda a: \sqcup \ \{\beta(f(c_i)) \ |\ c_i \sim \gamma(a)\}$\\
        $posConstraint \gets \lambda \abst{g}{}, \texttt{pexlst}: \forall \langle a, a' \rangle \in \texttt{pexlst}, (a' \sqsubseteq g^\#(a))$ \\
        $negConstraint \gets \lambda \abst{g}{}, \texttt{nexlst}: \forall \langle a, c' \rangle \in \texttt{nexlst}, (c' \notin \gamma(\abst{g}{}(a)))$ \\
%=======
%  \caption {\textsc{SynthesizeTransformer}($f$) // $C, A, \sqcup, \gamma, \alpha, \beta$\label{Alg:main}} % putting caption here at top, so \ref could work better
%  
%  
%  $posex, negex \gets \func{SampleExamples()}$ \\
%  $isSound, isPrecise \gets False$\\
%  $f^\sharp_{syn} \leftarrow \lambda a: \abst{\bot}{}$  \label{algo:absF} \\
%
%  \While{$\lnot isSound \lor \lnot isPrecise$} {
%    \label{Alg:main:outerwhile}
%    \If{$*$} { \label{Alg:main:if-nondet}
%      \If{$\lnot isSound$} { \label{Alg:main:sound}
%        $isSound, isPrecise, posex \gets \func{CheckSoundness}(\abst{f}{syn}, f, posex)$
%      }
%    }
%
%    \Else {
%      \If{$\lnot isPrecise$} { \label{Alg:main:precise}
%        $isSound, isPrecise, posex, negex \gets \func{CheckPrecision}(\abst{f}{syn}, posex, negex)$
%      }
%    }
%
%    \If{$\func{IsConsistent}(posex, negex)$} {
%      \label{Alg:main:consistent}
%      $\abst{f}{syn} \gets \func{GenTransformer}(\abst{f}{syn}, posex, negex)$
%    }
%    \Else {
%      $\abst{f}{syn}, posex, negex \gets \func{GenBestTransformer}(\abst{f}{syn}, posex, negex)$
%    }
%
%  }
%  \Return $f^\sharp_{syn}$
%\end{algorithm2e}
%
%\begin{algorithm2e}
%  \footnotesize
%  \DontPrintSemicolon
%  $\hat{f}^\sharp \gets \lambda a: \sqcup \ \{\beta(f(c_i)) \ |\ c_i \sim \gamma(a)\}$\\
%  $posConstraint \gets \lambda g^\sharp, \texttt{pexlst}: \forall \langle a, a' \rangle \in \texttt{pexlst}, (a' \sqsubseteq g^\sharp(a))$ \\
%  $negConstraint \gets \lambda g^\sharp, \texttt{nexlst}: \forall \langle a, c' \rangle \in \texttt{nexlst}, (c' \notin \gamma(g^\sharp(a)))$ \\
%>>>>>>> 43c4e41bf726e216cb2fdc9d9c9c3b566d1af7b1

  \caption {\textsc{Auxilliary Functions}}
\end{algorithm2e}

\begin{algorithm2e}
  \caption {\textsc{CheckSoundness}($\abst{f}{syn}, f, posex$)\label{Alg:checksound}}
  $res, \langle a, c \rangle \gets$ FuzzFind $a, c$, such that $c \in \gamma(a) \land f(c) \notin \gamma(f^\sharp_{syn}(a))$
  \label{algorithm:l:fuzz}
  
  \If{\textit{res} = \textsc{Success}} {
    $isPrecise \gets False$ \\
    $posex \leftarrow posex\ \cup \langle a, \hat{f}^\sharp(a) \sqcup \beta(f(c)) \rangle$
  }
  \Else {
    $isSound \gets True$ \label{algorithm:l:sound_t}
  }
  
  \Return $isSound, isPrecise, posex$
\end{algorithm2e}

\begin{algorithm2e}

  $f^\sharp_{old} \leftarrow \fSharpSyn$ \\
  $posConstraint \gets \lambda g^\sharp, \texttt{pexlst}: \forall \langle a, a' \rangle \in \texttt{pexlst}, (a' \sqsubseteq g^\sharp(a))$ \\
  $negConstraint \gets \lambda g^\sharp, \texttt{nexlst}: \forall \langle a, c' \rangle \in \texttt{nexlst}, (c' \notin \gamma(g^\sharp(a)))$ \\

  $res, f^\sharp_{syn}, \langle a, c' \rangle \gets SynthFind\ f^\sharp_{syn}, \langle a, c' \rangle \textrm{ such that }
  posConstraint(f^\sharp_{syn}, posex) \newline \hspace*{2cm}\land negConstraint(f^\sharp_{syn}, negex \cup \{ \langle a, c'\rangle \}) \newline
  \hspace*{2cm} \land c' \in \gamma(f^\sharp_{old}(a)) \setminus \gamma(f^\sharp_{syn}(a))$)\\ \label{algorithm:l:sketch}

  \If{res = Success}{
    $a' \gets \hat{f}^\sharp (a)$ \\  \label{algorithm:l:fhat}
    \If{$c' \in \gamma(a')$} {
      $isPrecise \gets False$\\
      $posex \gets posex \cup \{\langle a, a' \rangle\}$\\
    }
    \Else {
      $isSound \gets False$ \\
      $negex \gets negex \cup \{\langle a, c' \rangle\}$
    }
  }

  \Return $isSound, isPrecise, posex, negex$

  \caption {\textsc{CheckPrecision}($\abst{f}{syn}, posex, negex$)}
  \label{algorithm:algo}
\end{algorithm2e}

\begin{algorithm2e}
  \footnotesize
  \DontPrintSemicolon

  $res, f^\sharp_{syn} \gets SynthFind\ f^\sharp_{syn}  \textrm{ such that }$ \newline
  \hspace*{1.5cm} $posConstraint(f^\sharp_{syn}, posex) \land negConstraint(f^\sharp_{syn}, negex)$   \label{algorithm:l:sketchnocex}

  % $f^\sharp_{old} \leftarrow f^\sharp_{syn}$ \\

  % $res, f^\sharp_{syn}, \langle a, c' \rangle \gets SynthFind\ f^\sharp_{syn}, \langle a, c' \rangle \textrm{ such that }
  % posConstraint(f^\sharp_{syn}, posex) \newline \hspace*{2cm}\land negConstraint(f^\sharp_{syn}, negex \cup \{ \langle a, c'\rangle \}) \newline
  % \hspace*{2cm} \land c' \in \gamma(f^\sharp_{old}(a)) \setminus \gamma(f^\sharp_{syn}(a))$)\\ \label{algorithm:l:sketch}

  \Return $\abst{f}{syn}$

  \caption {\textsc{GenTransformer}($\abst{f}{syn}, posex, negex$)}
  \label{algorithm:algo}
\end{algorithm2e}


\begin{algorithm2e}
  \footnotesize
  \DontPrintSemicolon

  {
    \label{mainAlgo:maxsat}
    $\fSharpSyn, c,  dropnex \gets \textsc{SynthFindMax} \ \fSharpSyn \textrm{ such that } posConstraint(f^\sharp_{syn}, posex)|_{hard}\newline\hspace*{2.5cm} \land negConstraint(f^\sharp_{syn}, negex)|_{soft}$ \label{algorithm:l:sketchmaxsat}\\
    $posex \gets posex \cup \{\langle a, \beta(c')\rangle\ |\ \langle a, c' \rangle \in dropnex\}$ \label{algorithm:l:negtopops}\\
    $negex \gets negex \setminus dropnex$
  }

  \Return $\abst{f}{syn}, posex, negex$

  \caption {\textsc{GenBestTransformer}($\abst{f}{syn}, posex, negex$)}
  \label{algorithm:algo}
\end{algorithm2e}

\begin{algorithm2e}
  \footnotesize
  \DontPrintSemicolon
  $res, f^\sharp_{syn} \gets SynthFind\ f^\sharp_{syn}  \textrm{ such that }$ \newline
  \hspace*{1.5cm} $posConstraint(f^\sharp_{syn}, posex) \land negConstraint(f^\sharp_{syn}, negex)$   \label{algorithm:l:sketchnocex}

  \Return (\textit{res} = Success) ? $True$ : $False$ \label{algorithm:l:precise_t}

  \caption {\textsc{IsConsistent}($posex, negex$)}
  \label{algorithm:algo}
\end{algorithm2e}

\begin{algorithm2e}
  \footnotesize
  \DontPrintSemicolon

  $posex, negex \gets \emptyset$ \label{algo:posNegEx} \\
  $f^\sharp_{syn} \leftarrow \bot$  \label{algo:absF} \\
  $\hat{f}^\sharp \gets \lambda a: \sqcup \ \{\beta(f(c_i)) \ |\ c_i \sim \gamma(a)\}$\\
  $posex \gets \{\langle a, a'_p \rangle \ |\ a \sim A, a'_p\gets \hat{f}^\sharp(a) \}$ \\
  $negex \gets \{\langle a, c'_n \rangle \ |\ a \sim A, c' \notin \gamma(\hat{f}^\sharp(a))\}$\\
  $isSound, isPrecise \gets False$

  \While{$\lnot isSound \lor \lnot isPrecise$} {
    \label{algo:outerWhile}
    \If{$*$} { \label{algorithm:l:if}
      \If{isSound} {
        continue
      }
      $res, \langle a, c \rangle \gets$ FuzzFind $a, c$, such that $c \in \gamma(a) \land f(c) \notin \gamma(f^\sharp_{syn}(a))$
      \label{algorithm:l:fuzz}

      \If{\textit{res} = \textsc{Success}} {
        $isPrecise \gets False$
        $posex \leftarrow posex\ \cup \langle a, \hat{f}^\sharp(a) \sqcup \beta(f(c)) \rangle$
      }
      \Else {
        $isSound \gets True$ \label{algorithm:l:sound_t}
      }
    }

    \Else {
      \label{algorithm:l:else}
      \If{isPrecise} {
        continue
      }

      $f^\sharp_{old} \leftarrow f^\sharp_{syn}$ \\
      $posConstraint \gets \lambda g^\sharp, \texttt{pexlst}: \forall \langle a, a' \rangle \in \texttt{pexlst}, (a' \sqsubseteq g^\sharp(a))$ \\
      $negConstraint \gets \lambda g^\sharp, \texttt{nexlst}: \forall \langle a, c' \rangle \in \texttt{nexlst}, (c' \notin \gamma(g^\sharp(a)))$ \\

      $res, f^\sharp_{syn}, \langle a, c' \rangle \gets SynthFind\ f^\sharp_{syn}, \langle a, c' \rangle \textrm{ such that }
      posConstraint(f^\sharp_{syn}, posex) \newline \hspace*{2cm}\land negConstraint(f^\sharp_{syn}, negex \cup \{ \langle a, c'\rangle \}) \newline
      \hspace*{2cm} \land c' \in \gamma(f^\sharp_{old}(a)) \setminus \gamma(f^\sharp_{syn}(a))$)\\ \label{algorithm:l:sketch}

      \If{res = Success}{
        $a' \gets \hat{f}^\sharp (a)$ \\  \label{algorithm:l:fhat}
        \If{$c' \in \gamma(a')$} {
          $isPrecise \gets False$\\
          $posex \gets posex \cup \{\langle a, a' \rangle\}$\\
        }
        \Else {
          $isSound \gets False$
          $negex \gets negex \cup \{\langle a, c' \rangle\}$
        }
      }
      \Else { %{\textit{res} = Fail} \label{mainAlgo:nocexsat}
        % 
        $res, f^\sharp_{syn} \gets SynthFind\ f^\sharp_{syn}  \textrm{ such that }$ \newline
        \hspace*{1.5cm} $posConstraint(f^\sharp_{syn}, posex) \land negConstraint(f^\sharp_{syn}, negex)$   \label{algorithm:l:sketchnocex}

        \If{\textit{res} = Success} {
          $isPrecise \gets True$ \label{algorithm:l:precise_t}
        }

        \Else {
          \label{mainAlgo:maxsat}
          $f^\sharp_{syn}, c,  dropnex \gets \textsc{SynthFindMax} f^\sharp_{syn} \textrm{ such that } posConstraint(f^\sharp_{syn}, posex)|_{hard}\newline\hspace*{2.5cm} \land negConstraint(f^\sharp_{syn}, negex)|_{soft}$ \label{algorithm:l:sketchmaxsat}\\
          $posex \gets posex \cup \{\langle a, \beta(c')\rangle\ |\ \langle a, c' \rangle \in dropnex\}$ \label{algorithm:l:negtopops}\\
          $negex \gets negex \setminus dropnex$
        }
      }
    }

  }
  \Return $f^\sharp_{syn}$

  \caption {\textsc{SynthesizeTransformer}($f, A, \gamma, \alpha, \beta$)}
  \label{algorithm:algo}
\end{algorithm2e}

\subsection{Running Example}

Now we discuss the steps of the algorithm using a motivated example to synthesize an \textit{abstract transformer} for \texttt{abs(Int)} in interval domain (\textit{ID}).
% We will be using our algorithm to  synthesise abstract transformer for $abs()$ in interval domain.
Let the function to be synthesized be denoted as $f^\sharp_{syn}$ and is initlized to $\bot$ at line \ref{algo:absF}. \textit{posex} and \textit{negex} at line \ref{algo:posNegEx}, represents positive and negative sets of examples respenctively to synthesize $\fSharpSyn$.

For the synthesis process we start with concrete positive and negative examples provided by bootstrapping. The bootstrapping initializes the positive and negative example sets with following vlaues,
\begin{align*}
  & {posex_B} = \langle [-50, -41], [41, 50]\rangle, \langle [90, 100], [90, 100]\rangle, \langle [-40, -33], [33, 40] \rangle \\[1pt]
  &{negex_B} = \langle [-50, -41], 59\rangle, \langle [90, 100], 80\rangle, \langle [90, 100], 110\rangle, \langle [-40,-33], 26\rangle, \langle [-40, -33], 47\rangle
\end{align*}


% Bootstrap algorithm will give us following positive examples,\\ $\langle [-50, -41], [41, 50]\rangle$, $\langle [90, 100], [90, 100]\rangle$, $\langle [-40, -33], [33, 40]\rangle$.\\
% Following are some negative examples from our bootstrap algorithm.\\
% $\langle [-50, -41], \{32\}\rangle$, $\langle [-50, -41], \{59\}\rangle$, $\langle [90, 100], \{80\}\rangle$, $\langle [90, 100], \{110\}\rangle$, $\langle [-40, -33], \{26\}\rangle$, $\langle [-40, -33], \{47\}\rangle$-50, -41], \{32\}\rangle$, $\langle [-50, -41], \{59\}\rangle$, $\langle [90, 100], \{80\}\rangle$, $\langle [90, 100], \{110\}\rangle$, $\langle [-40, -33], \{26\}\rangle$, $\langle [-40, -33], \{47\}\rangle$.
% 

While loop at line.\ref{algo:outerWhile} iterates until both \textit{isSound} and \textit{isPrecise} are \textit{True}. In each iteration of the loop the algorithm takes a non-deterministic choice to improve the soundness or precision until the synthesized function $\fSharpSyn$ achieves both objectives or the program times out. We have shown below one execution instance of our algorithm for synthesizing abstract transformer for \texttt{abs()} function.



Let's in the firest iteration it starts with soundness check. Algorithm-\ref{algorithm:algo} asks the fuzzer a counterexample $a$ and $c$, such that $c \in \gamma(a) \land f(c) \notin \gamma(f_{syn}^\sharp(a))$ at line~.\ref{algorithm:l:fuzz}. Here, $f()$ is \texttt{abs()} and $f_{syn}^\sharp$ is $\bot$ in first iteration. Fuzzer gives, $[0, 11]$ as $a$ and $11$ for $c$, so $\langle [0, 11], [0, 11] \rangle$ is a new positive example.

\begin{align*}
  &posex = posex_B \cup \{\langle [0, 11], [0, 11] \rangle\}\\
  &negex = negex_B \cup \{\}
\end{align*}


In next iteration, algorithm takes say the \textit{else} block at line~\ref{algorithm:l:else}. Since \textit{isPrecise} is $False$, so algorithm invokes sketch to find a counterexample, $\langle a, c' \rangle$, and a function $f_{syn}^\sharp$, such that the following satisfied.
$$posConstraint(f^\sharp_{syn}, posex) \land        negConstraint(f^\sharp_{syn}, negex \cup \{ \langle a, c'\rangle \}) \land c' \in \gamma(f^\sharp_{old}(a)) \setminus \gamma(f^\sharp_{syn}(a))$$

Here, $f^\sharp_{old}(a)$ is $\bot$. Sketch produces $[25, 29]$ as $a$, and $0$ as $c'$.
$\hat{f}^\sharp$ produces $[25, 29]$ as $a'$. Since, $c' \notin \gamma(a')$, so $\langle [25, 29], \{0\} \rangle$ is a new negative example. In this iteration generated $f^\sharp_{syn}$ is as follows.

\begin{align*}
  &f^\sharp_{syn} \gets \lambda a : [max(a.l, -a.r),\ max(1-a.l, max(1, a.r))]\\
  &posex = posex_B \cup \{\langle [0, 11], [0, 11] \rangle\}\\
  &negex = negex_B \cup \{\langle [25, 29], 0 \rangle\}
\end{align*}


In next iteration, algorithm takes \textit{else} block at line~\ref{algorithm:l:else}. In this iteration, sketch produces, $[-15, -11]$ as $a$ and 15 as $c'$. Algorithm produces $[11, 14]$ as $a'$ at line no~\ref{algorithm:l:fhat}. In this case $c' \notin \gamma([11, 14])$, so it is considered as negative example. Generated $f^\sharp_{syn}$ is as follows.\\

\begin{align*}
  &f^\sharp_{syn} \gets \lambda a :[max(a.l, -a.r),\ a.l+a.r]\\
  &posex = posex_B \cup \{\langle [0, 11], [0, 11] \rangle\}\\
  &negex= negex_B \cup \{\langle [25, 29], \{0\} \rangle, \langle [-15, -11], \{15\} \rangle
\end{align*}

In 4$^{th}$ iteration, algorithm again uses sketch to find a counter example. This time sketch produces $\langle [-25, -21], \{20\} \rangle$ as negative example with following transformer.

\begin{align*}
  &f^\sharp_{syn} \gets \lambda a :[max(a.l, -a.r),\ max(max(0, a.r), \ -1-a.l)]\\
  &posex = posex_B \cup \{\langle [0, 11], [0, 11] \rangle\}\\
  &negex= negex_B \cup \{\langle [25, 29], \{0\} \rangle, \langle [-15, -11], \{15\} \rangle, \langle [-25, -21], \{20\} \rangle \}
\end{align*}


In 5$^{th}$ iteration, algorithm chooses \textit{else} block at line~.\ref{algorithm:l:else}, and sketch produce $\langle [-1, 3], -1\rangle$ as negative example. The generated function is

\begin{align*}
  &f^\sharp_{syn} \gets \lambda a :[max(max(0, a.l), -a.r),\ max(max(0, a.r), \ -1-a.l)]\\
  &posex = posex_B \cup \{\langle [0, 11], [0, 11] \rangle\}\\
  &negex= negex_B \cup \{\langle [25, 29], \{0\} \rangle, \langle [-15, -11], \{15\} \rangle, \langle [-25,-21], \{20\} \rangle, \langle [-1, 3], \{-1\}\rangle \}
\end{align*}


In 6$^{th}$ iteration, algorithm chooses \textit{True} for the condition at line~\ref{algorithm:l:if}. Fuzzer produced $[-1, 0]$ as $a$ and -1 as $c$. So $\langle [-1, 0], [0, 1] \rangle$ is a new positive example.

\begin{align*}
  &posex = posex_B \cup\{\langle [0, 11], [0, 11] \rangle, \langle [-1, 0], [0, 1] \rangle\}\\
  &negex= negex_B \cup \{\langle [25, 29], 0 \rangle, \langle [-15, -11], 15 \rangle, \langle [-25, -21], 20 \rangle, \langle [-1, 3], -1\rangle \}
\end{align*}

In next iteration, algorithm chooses sketch to find an example and a function. Sketch failed to provide an example and a function, $f_{syn}^\sharp$ at line no~\ref{algorithm:l:sketch}.
So algorithm tries to find a function which satisfy all positive examples and rejects all negative examples, at line no~\ref{algorithm:l:sketchnocex}. Sketch provides following function.\\

\begin{align*}
  &f^\sharp_{syn} \gets \lambda a :[max(-1+a.l,\  -a.r),\ max(-1-a.l,\  1+a.r)]\\
  &posex = posex_B \cup \{\langle [0, 11], [0, 11] \rangle, \langle [-1, 0], [0, 1] \rangle\}\\
  &negex= posex_B \cup \{\langle [25, 29], \{0\} \rangle, \langle [-15, -11], 15 \rangle, \langle [-25, -21], \{20\} \rangle, \langle [-1, 3], -1\rangle \}
\end{align*}



In next iteration, algorithm takes help from the fuzzer to find a counterexample. Fuzzer provided $[-60, 0]$ as $a$, and $c = -60$. $\langle [-60, 0], [0, 60] \rangle$ is another positive example.

\begin{align*}
  &posex =  posex_B \cup \{\langle [0, 11], [0, 11] \rangle, \langle [-1, 0], [0, 1] \rangle, \langle [-60, 0], [0, 60] \rangle\}\\
  &negex=  negex_B \cup \{\langle [25, 29], 0 \rangle, \langle [-15, -11], 15 \rangle, \langle [-25, -21], \{20\} \rangle, \langle [-1, 3], -1\rangle \}
\end{align*}


In 9$^{th}$ iteration, algorithm takes the help of sketch. Sketch provides a negative example $\langle [0, 4], \{5\} \rangle$ and following function.

\begin{align*}
  f^\sharp_{syn} \gets&~ \lambda a :[max(-1, a.l)*min(1, a.r),\ max(-1, a.r)-min(0, a.l)]\\
  posex = posex_B &\cup~ \{\langle [0, 11], [0, 11] \rangle, \langle [-1, 0], [0, 1] \rangle, \langle [-60, 0], [0, 60] \rangle\}\\
  negex = negex_B &\cup~ \{\langle [25, 29], \{0\} \rangle, \langle [-15, -11], \{15\} \rangle, \langle [-25, -21], \{20\} \rangle, \langle [-1, 3], \{-1\}\rangle\}\\ &\cup~\{ \langle [0, 4], \{5\} \rangle \}
\end{align*}



In next iteration also algorithm chooses to use sketch and sketch provides $\langle [-3, 1], \{-1\} \rangle$ as a new negative example and a new $f^\sharp_{syn}$ as follows,

\begin{align*}
  f^\sharp_{syn} \gets&~ \lambda a :[max(max(0, a.l)), \ -a.r]\\
  posex = posex_B &\cup~ \{\langle [0, 11], [0, 11] \rangle, \langle [-1, 0], [0, 1] \rangle, \langle [-60, 0], [0, 60] \rangle\}\\
  negex = negex_B &\cup~\{\langle [25, 29], \{0\} \rangle, \langle [-15, -11], \{15\} \rangle, \langle [-25, -21], \{20\} \rangle, \langle [-1, 3], \{-1\}\rangle\}\\ &\cup~\{ \langle [0, 4], \{5\} \rangle, \langle [-3, 1], \{-1\} \rangle \}
\end{align*}


In 11$^{th}$ iteration, algorithm chooses \textit{True} for the condition at line no~\ref{algorithm:l:if}. Fuzzer is able to find a counterexample, [-1, -1] as $a$ and -1 as $c$. So $\langle [-1, -1], [1, 1] \rangle$ added as positive example.

\begin{align*}
  posex =& posex_B~\cup \{\langle [0, 11], [0, 11] \rangle, \langle [-1, 0], [0, 1] \rangle, \langle [-60, 0], [0, 60] \rangle, \langle [-1, -1], [1, 1] \rangle\}\\
  negex =& negex_B \\ &\cup~\{\langle [25, 29], 0 \rangle, \langle [-15, -11], 15 \rangle, \langle [-25, -21], 20 \rangle, \langle [-1, 3], -1\rangle, \langle [0, 4], 5 \rangle, \langle [-3, 1], -1 \rangle \}
\end{align*}



In the next step, algorithm chooses sketch to find an example and a function at line no~\ref{algorithm:l:sketch}. In this step, sketch failed to get an example and a new function. So algorithm again tries to find a function which satisfy all positive examples and rejects all negative example at line no~\ref{algorithm:l:sketchnocex}. It is interesting to see that sketch also failed in this step.
This is only possible when there is conflict between positive and negative examples.
So we use sketch to solve a maxsat instance, where positive examples are hard constraints and negative examples are soft constraints at line no~\ref{algorithm:l:sketchmaxsat}. Sketch successfully produced a negative example $\langle [-2, 2], \{4\} \rangle$ and a new $f^\sharp_{syn}$ as follows.
$$f^\sharp_{syn} \gets \lambda a :[max(max(0, a.l), -a.r), \ max(-a.l, a.r)]$$

While doing maxsat, sketch dropped the negative example $\langle [-15, -11], \{15\} \rangle$ which was added in the third iteration. It was added in negative example as $\hat{f}^\sharp([-15, -11])$ gave [11, 14] as output and $c'= 15 \notin \gamma([11, 14])$. As it uses sampling while calculating $a'$, it misses the value 15. Though it was a positive example but it became a negative example.
Since maxsat dropped this negative example, so $\langle [-15, -11], \{15\} \rangle$ will be added to positive example at line no~\ref{algorithm:l:negtopops}.

\begin{align*}
  posex =& posex_B\\ &\cup~\{\langle [0, 11], [0, 11] \rangle, \langle [-1, 0], [0, 1] \rangle, \langle [-60, 0], [0, 60] \rangle, \langle [-1, -1], [1, 1] \rangle\} \\
         &\cup~\{ \mathbf{\color{red}\langle [-15, -11], [15, 15] \rangle}\} \\
  negex =& negex_B\\ & \cup~\{\langle [25, 29], 0 \rangle, \langle [-25, -21], 20 \rangle, \langle [-1, 3], -1\rangle, \langle [0, 4], 5 \rangle, \langle [-3, 1], -1 \rangle, \langle [-2, 2], 4 \rangle \}
\end{align*}


In the next step, sketch could not find a new example and a function at line no~\ref{algorithm:l:sketch}, but it succeed to find a function $f^\sharp_{syn}$, which satisfy positive example and rejects negative example at line no~\ref{algorithm:l:sketchnocex}. The variable \textit{isPrecise} is set to \textit{True} at line no~\ref{algorithm:l:precise_t}. Following is the new function generated in this step which is same as previous iteration.

\begin{align*}
  f^\sharp_{syn} \gets&~ \lambda a :[max(max(0, a.l), -a.r), \ max(-a.l, a.r)]\\
  posex =&~  posex_B\\ &\cup~\{\langle [0, 11], [0, 11] \rangle, \langle [-1, 0], [0, 1] \rangle, \langle [-60, 0], [0, 60] \rangle, \langle [-1, -1], [1, 1] \rangle \}\\ &\cup~\{ {\langle [-15, -11], [15, 15] \rangle}\}\\
  negex =&~ negex_B\\ &\cup~\{\langle [25, 29], \{0\} \rangle, \langle [-25, -21], \{20\} \rangle, \langle [-1, 3], \{-1\}\rangle, \langle [0, 4], \{5\} \rangle, \langle [-3, 1], \{-1\} \rangle \}\\ &\cup~\{ \langle [-2, 2], \{4\} \rangle \}
\end{align*}


In next iteration, fuzzer timeout to find a counterexample for last $f^\sharp_{syn}$, hence \textit{isSound} variable is updated to \textit{True} at line.~\ref{algorithm:l:sound_t}.
\begin{align*}
  posex =& \{\langle [0, 11], [0, 11] \rangle, \langle [-1, 0], [0, 1] \rangle, \langle [-60, 0], [0, 60] \rangle, \langle [-1, -1], [1, 1] \rangle\}\\ &\cup~\{ {\langle [-15, -11], [15, 15] \rangle}\}\\
  negex =& \{\langle [25, 29], \{0\} \rangle, \langle [-25, -21], \{20\} \rangle, \langle [-1, 3], \{-1\}\rangle, \langle [0, 4], \{5\} \rangle, \langle [-3, 1], \{-1\} \rangle\}\\ &\cup~\{ \langle [-2, 2], \{4\} \rangle \}
\end{align*}


Since both \textit{isSound} and \textit{isPrecise} is \textit{True}, so while loop terminates, and algorithm stops after producing following abstract transformer for concrete function $abs()$ which is sound and precise.\\
$$f^\sharp_{syn} \gets \lambda a :[max(max(0, a.l), -a.r), \ max(-a.l, a.r)]$$


==> slides/ai.tex <==

\begin{frame}[fragile]{Abstract Interpretation}
	\begin{minipage}{0.5\linewidth}    
		\begin{lstlisting}[language=C,numbers=left,xleftmargin=10pt,mathescape=true,escapechar=`]
int c = 42;		
while(*) {    `{\color{red}\only<2-4>{$c_{intv} = [42, 42]$}\only<5>{$c_{intv} = [42, 42] \sqcup [43,43]$}\only<6-8>{$c_{intv} = [42,43]$}\only<9>{$c_{intv} = [42, 43] \sqcup [44,44]$}\only<10>{$c_{intv} = [42,44]$}\only<11,12>{$c_{intv} = [42,\infty)$}}`
	c = c + 1;	`{\color{red}\only<3-4>{\color{red}$c_{intv} = [42,42] + [1,1]$}\only<7-8>{$c_{intv} = [43,43]+[1,1]$}\only<11-12>{\textsf{\small [widening]}}}`
}							`{\color{red}\only<4>{\color{red}$c_{intv}= [43,43]$}\only<8>{$c_{intv}=[44,44]$}}`
							`\only<12>{\color{red}$c_{intv} = [42, \infty)$}`
assert(c $\ge$ 42);
		\end{lstlisting}
	\end{minipage}
	\hfill
	\begin{minipage}{0.45\linewidth}
		\begin{tikzpicture}[remember picture, overlay]
		\only<3>{	\node[rectangle callout, draw=blue, fill=blue!10, align=center, callout absolute pointer={(-1,0.6)}] at (3.2,0.5) {$[l_1, r_1] +^\sharp [l_2, r_2] = [(l_1 + l_2), (r_1 + r_2)]$
%				\\[1em] $[42,42] +_{intv} [1,1] = [(42+1), (42+1)]$\\ \hspace*{1.05cm} $= [43,43] $
			};}
		\end{tikzpicture}
	\end{minipage}

%    \todo{show an AI run on this program}
%    \todo{put abstract operation in callout}
	
\end{frame}

\begin{frame}{Abstract Interpretation}
	\begin{tikzpicture}[remember picture, overlay]
		\only<1>{\node at (2,0) {\includegraphics[scale=.4]{fig/concDom1.pdf}};}
		\only<2->{\node at (2,0) {\includegraphics[scale=.4]{fig/concDom2.pdf}};}
		\node at (2, -3.4) {Concrete Domain};
		\node at (13,0) {\includegraphics[scale=.4]{fig/absDom.pdf}};
		\node at (13, -3.4) {Abstract Domain};
%		
%		\only<1,2>{
%			\node[rectangle callout, draw=red, fill=red!20, callout absolute pointer={(2.2, 1.8)}] at (6,0.5) {$10$};
%			
%			\node[rectangle callout, draw=red, fill=red!20, callout absolute pointer={(2.8, 0)}] at (6,-2) {$6$};
%			
%			\node[rectangle callout, draw=blue, fill=blue!20, callout absolute pointer={(13.6, 0.7)}] at (9,1) {$[6,10]$};
%		}
%		
%		\only<2>{
%			\node[rectangle callout, draw=red, fill=red!20, callout absolute pointer={(1.2, 0.5)}] at (0,2) {$7$};
%		}
%	
%		\only<3>{
%			\node[rectangle callout, draw=red, fill=red!20, callout absolute pointer={(3, -1.5)}] at (5,-2.5) {$2$};
%			
%			\node[rectangle callout, draw=red, fill=red!20, callout absolute pointer={(12.7, -1.5)}] at (9,-2.5) {$[2,2]$};
%		}
%		
		\draw[arrow,onslide=<2->{invisible}] (2.8,1.8)  to [bend left=30]  node[left, yshift=-0.8cm] {\only<1>{\LARGE$\mathbf{\alpha}$}} (13.8,0.9);
		
		\draw[arrow, onslide=<{1,3-}>{invisible}] (13.8, 0.5)  to [bend left=30] node[right, yshift=0.8cm, xshift=-1cm] {\only<2>{\LARGE$\mathbf{\gamma}$}}(3.2,0);
		
		
		
		\only<3>{
			\draw[arrow, onslide=<1>{invisible}] (3, -1.3)  to [bend left=30] node[left, yshift=-0.8cm, xshift=1cm] {\only<3>{\LARGE$\mathbf{\beta}$}}(12.5,-1.2);
		}
		
		
	\end{tikzpicture}
%    \todo{draw the actual points as in an example {1, 2, 5} -alpha-> [1,5] -gamma->{1,2,3,4,5}, put $\beta$ in figure, animate}
\end{frame}




==> slides/experiment.tex <==
\begin{frame}{Implementation and Experiments}
  \begin{itemize}
  \item<1-> \textsc{CheckSoundness}: Uses fuzz testing using the state-of-the-art fuzzer, AFL\footnote{\tiny AFL (american fuzzy lop), \href{https://lcamtuf.coredump.cx/afl/}{https://lcamtuf.coredump.cx/afl/}}
    
  \item<2-> \textsc{CheckPrecision}: Uses the program synthesizer, Sketch\only<2>{\footnote{\tiny A. Solar-Lezama, ``Program sketching'', in STTT'13}}
  \end{itemize}
  \pause

\end{frame}



\begin{frame}{Research Questions}
    \begin{enumerate}
    \item Can \tool synthesize sound and precise abstract transformers?
    \pause
    	\begin{itemize}
    		\item We did manual inspection to check soundness and precision of abstract transformers.
    	\end{itemize}
    \pause
    \item How do the transformers synthesized by \tool compare to manually written ones?
\begin{itemize}
    \item  We \textit{replaced} the manually-written abstract transformers in in a state-of-the-art verifier (\safestr\footnote{\tiny R. Amadini, A. Jordan, G. Gange, F. Gauthier, P. Schachte, H. Søndergaard, P. J. Stuckey \& C. Zhang, ``Combining String Abstract Domains for JavaScript Analysis: An Evaluation'', in TACAS’17}) by our synthesized ones; \safestr is a state-of-art static analyzer to analyze complex string operations for JavaScript web applications.
    	\pause
    \item Each benchmark was run on \safestr instantiated with the manual and synthesized sets of transformers; we measured
    	\begin{itemize}
    		\item time taken
    		\item number of fixpoint iterations of the analysis
    		\item number of reachable program states
    		\item imprecision index
    	\end{itemize}
\end{itemize}
%    \pause
    \end{enumerate}

\end{frame}

\begin{frame}{Time taken to synthesize}
\begin{table}
	%		\centering
	
	\begin{tabular}{l|rrrrr}
		& $\csdom$ & $\ssk$ & $\charin$ & $\psdom$ & $\mathcal{SH}$\\
		\hline
		\texttt{charAt}   & 615 & 616 & 1442 & 674 & n/a \\
		\texttt{concat}   & 640 & 624 & 1953 & 621 & 657 \\
		\texttt{contains} & 657 & 765 & 1218 & 622 & n/a \\
		\texttt{toLower}  & 615 & 617 & 781  & 613 & n/a \\
		\texttt{trim}     & 615 & 622 & 713 & 616 & n/a \\
		\texttt{toUpper}  & 611 & 622 &  625 & 613 & n/a
	\end{tabular}
	\caption{Time, in seconds, to synthesize abstract transformers for string functions.
	}
\end{table}
\end{frame}


\begin{frame}[fragile]{Comparison with manual operations}
\begin{figure}
	\includegraphics[scale=0.3]{./fig/result_coci.pdf}
	\caption{Performance with the product domain $\csdom \times \charin$.}
	
	\label{Fi:CharInEvaluation}
\end{figure}

\end{frame}

\begin{frame}{Character Inclusion ($\charin$)\footnote{Magnus Madsen and Esben Andreasen, ``String analysis for dynamic field access'' In CC 2014}}

	  	\begin{itemize}
	  		\item $\charin = \{\bot_{\charin}\} \cup \{\left[L,U\right] \mid   L, U \subseteq \Sigma, L \subseteq U\}$	
	  		\pause
	  		\item $L:$ \textit{must} set\\ $U:$ \textit{may} set
	  		\pause
	  		\item $\alpha_\charin(\{s_1,\ldots,s_n\})=[\bigcap_i char(s_i),\bigcup_i char(s_i)]$
	  		\pause
	  		\item $\gamma_\charin([L,R])=\{s\mid   L\subseteq char(s)\subseteq R \}$
	  		\pause
	  		\item $[L_1, U_1] \sqsubseteq_\charin [L_2, U_2] \Leftrightarrow (L_1 \subseteq L_2 \land U_1 \subseteq U_2)$
	  	\end{itemize}
	  	
\end{frame}

\begin{frame}{\texttt{contains} in $\charin$}
%  \todo{give language and domain description, show the bug via a callout}
 
  \only<1>{
  	\tikz[remember picture, overlay]{
  		\node[rectangle, draw=red, fill=aliceblue, align=center, rounded corners=2pt] at (8,0.5) {\ttfamily contains(str1, str2) $=\begin{cases}
  			\top & \textrm{if \texttt{str2} is substring of \texttt{str1}}\\
  			\bot & \textrm{otherwise}
  			\end{cases}$
  		};
  	}
	  \begin{align}
	  \textit{Transformer} ::= &\ \lambda \mathtt{a_1,a_2} . AB \nonumber\\
	  AB ::=&\ \texttt{ite}(B, AB, AB) \mid \texttt{BoolTop}\mid  \texttt{BoolBot}\mid  \texttt{BoolTrue}\mid  \texttt{BoolFalse} \nonumber\\
	  B ::=&\ \texttt{isSubset}(LU, LU)\mid  \texttt{size}(LU) \leq 1\mid  \texttt{size}(LU) = 0\mid  \texttt{isBot}(CI) \nonumber\\
	  \mid&\ \texttt{isTop}(CI)\mid  \neg B\mid   B\land B\mid   B\lor B \nonumber\\
	  CI ::= &\ \mathtt{a_1} \mid \mathtt{a_2}  \nonumber\\
	  LU ::=&\ CI.\texttt{l}\mid  CI.\texttt{u} \nonumber
	  \end{align}
  }
  
  \only<2->{
  	
  \begin{figure}
  	\vspace{-1cm}
    \scalebox{.8}{
      \begin{minipage}{.6\linewidth}
          \caption*{\Large Original (buggy) transformer in \safestr}
	\lstinputlisting[language=C,numbers=left, escapechar=@]{code/containsSafe.pk}
	
    \end{minipage}}%%
    \hfill
    \scalebox{.8}{
      \begin{minipage}{.55\linewidth}
	\caption*{\Large Synthesized abstract transformer}
	\lstinputlisting[language=C,numbers=left,escapechar=@,mathescape]{code/containsSketch.pk}
	
	\vspace{3ex}
    \end{minipage}}
%    \caption*{Abstract transformers for \texttt{contains} in the $\charin$ domain.}
  \end{figure}

%	\tikz[remember picture, overlay]{
%		\node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=0.5,minimum width=5cm, rounded corners=2pt, minimum height=2cm,inner ysep=1em, callout absolute pointer={(6,3)}] at (9,6.5) {\LARGE In $\charin$ \texttt{boolTrue}, is unsound verdict for \texttt{contains}};
%	}
  }
  
  \uncover<3>{
		\tikz[remember picture, overlay]{
            \node[rectangle, draw=red, fill=aliceblue, align=center, rounded corners=2pt] at (7,-0.3) {\texttt{$s_1$=\{"aa"\}, $s_2$=\{"aaaaa"\}}\\ \texttt{$a_1$=[\{`a'\}, \{`a'\}], $a_2$=[\{`a'\}, \{`a'\}]}
				%\texttt{contains(str1, str2) $\notin \gamma(\mathtt{contains}^\sharp(\mathtt{absStr1}, \mathtt{absStr2}))$}
				};
		}
%		\fcolorbox{red}{aliceblue}{x}
	 }
	 
\end{frame}

\begin{frame}{\texttt{trim} in $\charin$}
%  \todo{give language and domain description}
%  \todo{why a white line on the second figure?(pk: have to look into it)}

	\only<1->{
	\tikz[remember picture, overlay]{
		\node[rectangle, draw=red, fill=aliceblue, align=center, rounded corners=2pt] at (7.5,.5) {{\ttfamily trim(str)} = returns a string after removing \\\hspace*{1cm} leading and trailing spaces from \texttt{str}};
	}	
	}
  \only<1>{
	  \begin{align}
	  \textit{Transformer} ::= &\ \lambda \texttt{a} . CI \nonumber\\
	  CI::=&\ \texttt{a}\mid [\emptyset, \emptyset] \mid [LU, LU]\mid \texttt{ite}(B, CI, CI) \nonumber\\
	  B::=&\ \texttt{size}(LU) \leq 1\mid  \texttt{size}(LU) = 0\mid  \texttt{isBot}(CI)\nonumber\\
	  |&\ \texttt{isTop}(CI)\mid  \texttt{containsSpace}(LU)|\ \neg B\mid   B\land B\mid   B\lor B \nonumber\\
	  LU ::=&\ CI.\texttt{l}\mid  CI.\texttt{u}\mid  \texttt{removeSpace}(LU)\nonumber
	  \end{align}	
  }
  \only<2>{
  	\tikz[remember picture, overlay]{
  		\node[rectangle, draw=red, fill=aliceblue, align=center, rounded corners=2pt] at (7,-5) {\ttfamily
%  			\LARGE In  \texttt{trim}, \textit{must} set will not have space in $a'$

            strs = \{"\textvisiblespace \textvisiblespace abc\textvisiblespace \textvisiblespace", "a\textvisiblespace a"\}	\\[1mm]
			$a$ = [\{`\textvisiblespace',`a'\}, \{`\textvisiblespace',`a',`b',`c'\}]\\[1mm]
            $\abst{trim}{}(a)$ = [\{`a'\}, \{`\textvisiblespace',`a',`b',`c'\}]
			%trim(str) $\notin \gamma$(trim$^\sharp$(absStr))
  			};
  	}
  \begin{figure}
    \scalebox{.72}{
      \begin{minipage}{.65\linewidth}
          \caption*{\Large Original (buggy) transformer in \safestr}
	\lstinputlisting[language=C,numbers=left, escapechar=|]{code/trimSafe.pk}
	\vspace*{6ex}
    \end{minipage}}%%
    \hfill
    \scalebox{.72}{
    	
      \begin{minipage}{.65\linewidth}
      	\caption*{\Large Synthesized abstract transformer}
	\lstinputlisting[language=C,numbers=left,escapechar=|]{code/trimSketch.pk}
       \vspace*{6ex}
    \end{minipage}}
%    \caption{Abstract transformers for \texttt{trim} in the $\charin$ domain.}
  \end{figure}
 }
\end{frame}

\begin{frame}{String Hash ($\mathcal{SH}$)\footnote{Magnus Madsen and Esben Andreasen, ``String analysis for dynamic field access'' In CC 2014}}
	\begin{itemize}
		\item A fixed-size universe $U = \{0,\dots,b-1\}$ 
		\pause
		\item Hash function, $h(s) = (\Sigma_{c \in char(s)}I(c))~mod~b$, where $I:\Sigma \rightarrow \mathbb{N}$ (e.g., ASCII value of characters) 
		\pause
		\item $\alpha_\mathcal{SH}(S) = \{ h(s) \mid s \in S \}$
		\pause
		\item $\gamma_{\mathcal{SH}} (H) = \{s \in \Sigma^* \mid   h(s) \in H\}$
	\end{itemize}
\end{frame}


\begin{frame}{\texttt{concat} in $\mathcal{SH}$}
%  \todo{give language and domain description}


\only<1>{
  \begin{figure}
    \scalebox{.9}{
      \begin{minipage}{.5\linewidth}
	\lstinputlisting[language=C,numbers=left, escapechar=@]{code/hashSafe.pk}
	
	%			\subcaption{Abstract transformer in \safestr}
    \end{minipage}}%%
    \hfill
    \scalebox{.9}{
      \begin{minipage}{.5\linewidth}
	\lstinputlisting[language=C,numbers=left,escapechar=@]{code/hashSketch.pk}
	
	%					\vspace{3ex}
	%			\subcaption{Synthesized abstract transformer}
    \end{minipage}}
    \caption{Abstract transformers for \texttt{concat} in the $\mathcal{SH}$ domain.}
  \end{figure}
  }
\end{frame}





\begin{frame}[fragile]{Conclusions}

  \begin{itemize}
  \item Verification of ``real" programs requires reasoning over constructs that cannot be anslyzed using symbolic techniques (black-box operations)
    \pause
  \item Current techniques at handling such operations are either highly imprecise, unsound, or manual and error-prone.
    \pause
  \item Our tool, \tool, is capable of automatically synthesizing non-trivial abstract transformers, enabling verification over programs using such blck-box operations.
    \pause
  \item Our experiments on the \safestr tool shows the value of such an endevour.
  \end{itemize}

\end{frame}

\begin{frame}
	\only<1>{\centering
		\scalebox{.5}{
			\lstinputlisting[language=C,numbers=left, escapechar=@]{../code/hashDSLSketch.sk}	
		}
	}
\end{frame}



==> slides/maxsat.tex <==
\begin{frame}{Building the oracles...}
%    \todo{add examples}
    
	\tikz[remember picture, overlay]{
	\uncover<2-3>{
		\node[ellipse callout, draw=red, fill=blue!20, inner sep=2pt, align=center,aspect=8,cloud puffs=50,cloud puff arc=100,anchor=center,  minimum width=3cm, callout absolute pointer ={(5.5,-1)}, align=center] at (11,1) {
			%\only<2>{$\abst{\widehat{f}}{}(a)$ is not available!}\\
            %\only<2>{\Large \textbf{?}}
            \only<2>{?}
             \only<3>{$\gamma(\abst{\widehat{f}}{}(a)) \equiv \{\llbracket {f(c)} \rrbracket \ | \ c \in \gamma(a) \}$}	
			
		};
	}
		
		
%	\uncover<3->{
%		\node[rectangle ,draw=red, fill=darkmagenta!20,inner sep=2pt,align=center,aspect=2,scale=0.7,minimum width=5cm, rounded corners=2pt, minimum height=2cm,inner ysep=1em] at (12,0) {\Large
%            {$\abst{\widehat{f}}{L}$ is not known!}
%			%\\\Large 			\only<4>{Solution: approximate the best L-transformer by $\abst{f}{E}$, s.t.,\\\LARGE 				$\forall \B{a,c} \in \pex \, .~c \in \gamma(\abst{f}{E}(a)) \land$\\\LARGE$ \forall \B{a,c} \in \nex \, .~c \not\in \gamma(\abst{f}{E}(a))$}
%			};
%		}	
%	}
	
	\uncover<5-6>{
		\tikz[remember picture, overlay]{
            \node[ellipse callout, draw=red, fill=blue!20, inner sep=2pt, align=center,aspect=8,cloud puffs=50,cloud puff arc=100,anchor=center,  callout absolute pointer ={(8.6,-4)}, align=center] at (12,-1) {
                \only<5>{?}
            	%\only<6-> {$\abst{\widehat{f}}{L}$ is not known!}\\
            	\only<6>{$\abst{\widehat{f}}{L} \equiv \abst{\widehat{f}}{E}$}
            	};
		}
	}	
	}

    \begin{itemize}
	   %\item Let $\abst{f}{E} \gets \lambda a.[a.l, a.r]$, be a transformer 
  	
	   %\pause  	
       \item {\bf CheckSoundness} requires the following check:
       
       \begin{itemize}
       	
       \item $\langle a,c'\rangle$ such that $c' \in \gamma(\abst{\hat{f}}{}(a)) \setminus \gamma(\abst{f}{E}(a))$
       
       %\pause \pause
       
	   %\item $ \exists \B{a,c'}, a \in A, c' \in C, \textrm{ such that } \exists c \in C, c \in \gamma(a) \land c'= \llbracket f(c) \rrbracket \land c' \notin \gamma(\abst{f}{E}(a))$
   
	   %\pause
	   
	   %${\color{red}\B{[-4, 0], 3}}$ is a soundness counterexample for $\abst{f}{E}$
	   
		\end{itemize}
		
		\vspace{2cm}
	   
	   
	   \item<4-> {\bf CheckPrecision} requires the following check:
	   \begin{itemize}
	     
	     \item $\langle a,c'\rangle$, if $\exists \langle a,c'\rangle $, such that $c' \in \gamma(\abst{f}{E}(a)) \setminus \gamma(\abst{\hat{f}}{L}(a))$
	     
	     %\pause\pause
	     
	     %\item $\exists \abst{h}{L}, \langle a, c' \rangle. sat^+(\abst{h}{L}, \pex)  \land sat^-(\abst{h}{L}, \nex \cup \{ \langle a, c'\rangle \}) \nonumber \land \neg sat^-(\abst{f}{E}, \{ \B{a, c'} \})$\\
          
	      %\pause
	      
	      %${\color{blue}\B{[-4, 0], 5}}$ is a precission counterexample
    \end{itemize}
      
%       \todo{add check and add a callout that $\widehat{\abst{S}{L}}$ is not known, Solution: approximate the best L-transformer by $\abst{f}{E}$}
  \end{itemize}
\end{frame}

\begin{frame}{Failed consistency}
%  \begin{center}
%\tikz[remember picture, overlay]{
%	\node at (7,0) {
  	\hspace*{3cm}\only<1>{\includegraphics[scale=.8]{fig/0_1.pdf}}
	\hspace*{-.13cm}\only<{2}>{\includegraphics[scale=.8]{fig/0.pdf}}
    \hspace*{-.13cm}\only<3>{\includegraphics[scale=.8]{fig/1.pdf}}
    \hspace*{-.13cm}\only<{4,5}>{\includegraphics[scale=.8]{fig/2.pdf}}
    \hspace*{-.13cm}\only<6>{\includegraphics[scale=.8]{fig/3.pdf}}
	\hspace*{-.13cm}\only<7>{\includegraphics[scale=.8]{fig/4.pdf}}
%	};
%}
%  \end{center}

  \tikz[remember picture, overlay]{
      \node at (8,-.5 ) {\only<5>{\fcolorbox{red}{darkmagenta!20}{Inconsistent: no $\abst{f}{E} \in L$ that satisfies all positive and negative examples.}}};
    \node at (8,-.5) {\only<6->{\fcolorbox{red}{darkmagenta!20}{Occam's razor}}};
  }
\end{frame}

\begin{frame}{Modified algorithm}
%    \todo{provide callouts for the interfaces}
  \tikz[remember picture,overlay,pin distance=0cm]{
%    \begin{scope}[on background layer]
      \draw[fill=red!40,rectangle,rounded corners] (2.2,1.7) rectangle (7.5,2.1);	
      \draw[fill=red!40, rectangle,rounded corners] (2.2,.35) rectangle (7.5,1.05);
%    \end{scope}

	\uncover<2->{
		\node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=0.5,minimum width=5cm, rounded corners=2pt, minimum height=2cm,inner ysep=1em, callout absolute pointer={(7.5,1.9)}] at (12,2) {\LARGE$\  \exists \abstfe.\ sat^+(\abstfe, \pex) \land sat^-(\abstfe, \nex)\ $};
	}

	\uncover<3->{
		\node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=0.5,minimum width=5cm, rounded corners=2pt, minimum height=2cm,inner ysep=1em, callout absolute pointer={(7.5,.9)}] at (12,0) {\LARGE $\exists \abst{f}{E}, D. \  sat^+(\abst{f}{E}, \pex)  \land sat^-(\abst{f}{E \setminus D}, \nex)$,\\ \LARGE\textit{where $D$ is minimal set}};
	}
	
  }
  \scalebox{.6}{
    \hspace*{3cm}
    \begin{algorithm2e}[H]
      \setcounter{algocf}{1}
      \caption {\textsc{SynthesizeTransformer}($f$) // $C, A, \sqcup, \gamma, \alpha, \beta, L$\label{Alg:main}}
      
      $\abst{f}{E} \leftarrow \lambda a: \bot$\\
      $isSound, isPrecise \gets False$\\
      $\pex, \nex \gets \func{InitializeExamples()}$ \label{Alg:main:sampling}
      
      \While{$\lnot \textit{isSound} \lor \lnot \textit{isPrecise}$} {      \label{Alg:main:outerwhile}

	\tikzmark{s1}\If{$\func{CheckConsistency}(\pex, \nex)$} {\tikzmark{e1}   
	  \label{Alg:main:isconsistent}
	  $\abst{f}{E} \gets \func{Synthesize}( \pex, \nex)$ \label{Alg:main:gentransformer}
	}
	\tikzmark{s2}\Else {
	  $\abst{f}{E}, \delta \gets \func{MaxSatSynthesize}( \pex, \nex)$\\
	  %$\pex \gets \pex \cup \delta$\\
	  $\nex \gets \nex \setminus \delta$
	}\tikzmark{e2}
	\If{$*$} { \label{Alg:main::if-nondet}
	  
	  { \label{Alg:main:sound}
	    %              \twr{Why does $\func{CheckSoundness}$ set $\textit{isPrecise}$?} \\
	    $\textit{isSound}, e \gets \func{CheckSoundness}(\abst{f}{E}, f, \pex, \nex)$\\
	    \If{$\lnot \textit{isSound}$}{
	      {$\textit{isPrecise} \gets \bot$}\\
	      $\pex \gets \pex \cup \{e\}$ \label{Alg:main:AdjustEPlus}
	    }
	  }
	}
	
	\Else {
	  
	  { \label{Alg:main:precise}
	    %               \twr{Why does $\func{CheckPrecision}$ set $\textit{isSound}$?} \\
	    $\textit{isPrecise}, e \gets \func{CheckPrecision}(\abst{f}{E}, \pex, \nex)$\\
	    \If{$\lnot isPrecise$}{
	      {$\textit{isSound} \gets \bot$}\\
	      $\nex \gets \nex \cup \{e\}$ \label{Alg:main:AdjustEMinus}
	    }
	  }
	}
	
      }
      \Return { $\abst{f}{E}$ }
    \end{algorithm2e}
  }
 

\end{frame}

\begin{frame}{Claims}
    \begin{theorem}
		If Algorithm terminates, it returns a best $L$-transformer for the concrete function $f$.
	\end{theorem}
	
	\begin{theorem}
		If the DSL $L$  is finite, Algorithm always terminates.
	\end{theorem}
\end{frame}

\begin{frame}{Summary of our algorithm}
	\centering
	\includegraphics[scale=.35]{../fig/cegis-loops.pdf}
\end{frame}


==> slides/motivation.tex <==

\begin{frame}{Abstract Interpretation with Black-Box operations}	
  \begin{center}
    
    \begin{minipage}{.5\linewidth}
      \hspace*{3cm}
      \scalebox{.8}{\lstinputlisting[language=C,numbers=left]{code/moti.c}}
    \end{minipage}
  \end{center}
  \uncover<2->{
    \tikz[remember picture,overlay]{
      \node[rectangle callout,draw=red, fill=mymauve!30,inner sep=2pt,align=center,aspect=2,scale=0.5,minimum width=3cm, minimum height=1cm,inner ysep=1em,rounded corners=2pt, callout absolute pointer={(9.5,1.5)}] at (12,2) {\LARGE foo $\equiv$ Math.abs};
      
      %%change callout absolute pointer to change the arrow head
      
      %			\node[ rectangle,draw, fill=mymauve!30 ,align=center, rounded corners=2pt] at (12 ,1.6) (aa) {
      %                foo $\equiv$ abs	};
    }
  }
  \uncover<3->{
    \begin{block}{Possible solutions}

      \begin{itemize}
      \item<4-> \only<4->{Overapproximation}  \only<5->{ --- high false positive rate}
      \item<6-> \only<6->{Underapproximation heuristics\footnote{\tiny A. Das, S. Lahiri, A. Lal, and Y. Li, ``Angelic verification: Precise verification modulo unknowns,'' in CAV'15}}  \only<7->{--- missed bugs}
      \item<8-> \only<8->Provide stubs \only<9->{--- difficult manual task, error-prone}
      \end{itemize}

    \end{block}
  }
  %        \todo{animate slide}

\end{frame}







==> slides/oracle_star.tex <==

\begin{frame}{\tool in action!}

	\tikz[remember picture,overlay]{
		
%		\node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=0.5,minimum width=5cm, rounded corners=2pt, minimum height=2cm,inner ysep=1em, callout absolute pointer={(6.5,1.4)}] at (10,1.8) {\LARGE$\begin{cases}
%			\abst{f}{E}  &\textrm{if}~\exists \abstfe.\ sat^+(\abst{f}{E}, \pex) \land sat^-(\abst{f}{E}, \nex)\\
%			\bot &\textrm{otherwise}
%			\end{cases}$};
		
%		\only<2>{
%            \node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=1,minimum width=5cm, rounded corners=2pt, minimum height=2cm,inner ysep=1em, callout absolute pointer={(8.8,-.5)}] at (12,3) {\textbf{Positive example}: \\$\langle a,c'\rangle$ s.t. $a\in A$ and $c'\in \gamma(\abst{\hat{f}}{}(a))$};
%		}
%		
%		\only<4>{
%            \node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=1,minimum width=5cm, rounded corners=2pt, minimum height=2cm,inner ysep=1em, callout absolute pointer={(13,-1.5)}] at (3,3) {\textbf{Negative example}: \\$\langle a,c'\rangle$ s.t. $a\in A$ and \\ $c'\notin \gamma(\abst{\hat{f}}{L}(a))$ for some $\abst{\hat{f}}{L} \in \abst{\hat{\mathcal{S}}}{L}$};
%		}

		\only<1>{
            \node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=1,minimum width=1cm, rounded corners=2pt, minimum height=1cm,inner ysep=1em, callout absolute pointer={(8.5,0)}] at (12,3) {$\abst{f}{abs} \gets \lambda a.[0,2]$};
		}

		\only<2>{
            \node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=1,minimum width=5cm, rounded corners=2pt, minimum height=2cm,inner ysep=1em, callout absolute pointer={(8.8,-.5)}] at (12,3) {$\abst{f}{abs} \gets \lambda a.[0,2]$ \\ \textbf{Positive counterexample}: $\B{[0,5], 3}$ };
		}
	
		\only<3>{
			\node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=1,minimum width=1cm, rounded corners=2pt, minimum height=1cm,inner ysep=1em, callout absolute pointer={(3.5,0)}] at (2,3) {$\abst{f}{abs} \gets \lambda a.[0, a.l + a.r]$};
		}
		
		\only<4>{
            \node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=1,minimum width=5cm, rounded corners=2pt, minimum height=2cm,inner ysep=1em, callout absolute pointer={(13,-1.5)}] at (3,3) { $\abst{f}{abs} \gets \lambda a.[0, a.l + a.r]$ \\ \textbf{Negative counterexample}: $\B{[3,7], 8}$};
		}

		%	\centering
		%circles
		\draw[ onslide=<{1,2}>{base}, onslide=<{3-}>{invisible}](7.5,0) ellipse (1 and .5);%1 smaller one
		
		\draw[ onslide=<{1,2,3,4}>{invisible},onslide=<{5,6}>{base}, onslide=<{7-}>{invisible}](7.5,0) ellipse (2 and 1);%2
		
		\draw[ onslide=<9>{base}, onslide=<{-8}>{invisible}](8,0) ellipse (3 and 1.5);%5
		
		\draw[color=black, thick, dashed](8,0) ellipse (3.5 and 1.8); %f_l^#
		\node at (8,2.3) {\LARGE$\abst{\widehat{f}}{L}$};
		
		\draw[ onslide=<{7,8}>{base}, onslide=<{1-6}>{invisible}, onslide=<9>{invisible}](8.2,0) ellipse (4.3 and 2.2);%4
		
		\draw[ onslide=<{1,2}>{invisible},onslide=<{3,4}>{base}, onslide=<{5-}>{invisible}](9,0) ellipse (5.5 and 3); %3 bigger one
		
		%dots
%		\node at (7.5,0) (a) {\textcolor{green!70!blue}{$\bullet$}}; % most inside one
		\node[onslide=<2->{}, onslide=<1>{invisible}] at (8.8,-.5) (a) {\only<2>{\textcolor{green!70!blue}{$\bigstar$}} \only<3->{\textcolor{green!70!blue}{$\bullet$}}};
		
		\node[onslide=<6->{}, onslide=<{1-5}>{invisible}] at (9.8,.5) (a) {\only<6>{\textcolor{green!70!blue}{$\bigstar$}} \only<7->{\textcolor{green!70!blue}{$\bullet$}}};
		
		\node[onslide=<8->{}, onslide=<{1-7}>{invisible}] at (11.8,0) (a) {\only<8>{\textcolor{red}{$\bigstar$}} \only<9->{\textcolor{red}{$\bullet$}}};
		
		\node[onslide=<1-3>{invisible}, onslide=<4>{}] at (13,-1.5) (a) {\only<4>{\textcolor{red}{$\bigstar$}} \only<5->{\textcolor{red}{$\bullet$}}};
		
		%label
%		\node at (5,-4) {\textcolor{green!70!blue}{$\bigstar$}: positive counterexample, \textcolor{red}{$\bigstar$}: negative counterexample};
%		\node at (5,-4.5) {\textcolor{green!70!blue}{$\bullet$}: positive example, \textcolor{red}{$\bullet$}: negative example};

		    \node[rectangle, fill=yellow!20, draw=yellow] at (7,-3.5){Simplifying assumption: $\abst{\widehat{f}}{L} = \abst{\widehat{f}}{}$};
	}
	
	%    \todo{add the ideal transformer, remove the intermediate transformers}
\end{frame}

\begin{frame}{Algorithm Overview}

    \begin{itemize}
        \item \tool uses counterexample-guided inductive synthesis (CEGIS) synthesis strategy;
			\pause	
        \item attempts to meet the dual objectives of soundness and precision;
			\pause	
        \item correspondingly, the algorithm is guided by two kinds of examples
        	\pause
%            \todo{callout for S and $f_E$}
	\begin{itemize}
		\item \textbf{positive examples} ($E^+$): $\langle a,c'\rangle$ such that, $a\in A$ and $c'\in \gamma(\abst{\hat{f}}{}(a))$\\
            e.g., $\langle[5, 9], 6 \rangle$ ($abs$ in interval domain)
			\pause
		\item \textbf{negative example} ($E^-$): $\langle a,c'\rangle$ such that, $a\in A$ and $\exists\ \abst{\hat{f}}{L} \in \abst{\hat{\mathcal{S}}}{L}$ such that, $c'\notin \gamma(\abst{\hat{f}}{L}(a))$\\
            e.g., $\langle[5, 9], 2 \rangle$ ($abs$ in interval domain)
	\end{itemize}
	
	\pause
\item counterexamples generated by the \textbf{soundness} and \textbf{precision} oracles
%	\pause
%    \begin{itemize}
%        \item \textsc{CheckSoundness*}: Takes an $L$-transformer $\abst{f}{E}$ and returns,
%        \pause
%	\begin{itemize}
%		\item \texttt{False}, $\langle a,c'\rangle$, if $\exists \langle a,c'\rangle$, such that $c' \in \gamma(\abst{\hat{f}}{}(a)) \setminus \gamma(\abst{f}{E}(a))$ (\textit{positive counterexample});
%		\pause
%        \item \texttt{True}, if $\forall a. \abst{\hat{f}}{}(a) \sqsubseteq \abst{f}{E}(a)$;
%        \pause
%	\end{itemize}
%        \item \textsc{CheckPrecision*}: Takes an $L$-transformer $\abst{f}{E}$ and returns,
%        \pause
%	\begin{itemize}
%        \item \texttt{False}, $\langle a,c'\rangle$, if $\exists \langle a,c'\rangle $, such that $c' \in \gamma(\abst{f}{E}(a)) \setminus \gamma(\abst{\hat{f}}{L}(a))$, where, $\abst{\hat{f}}{L}$ is a best $L$-transformer (\textit{negative counterexample});
%        \pause
%		\item \texttt{True}, otherwise. 
%	\end{itemize}
%    \end{itemize}
    \end{itemize}

\end{frame}


\begin{frame}{Algorithm}
%    \todo{callout for CheckSoundness and CheckPrecision}
	 \tikz[remember picture,overlay,pin distance=0cm]{
	 
	 	\uncover<2->{
	 		\node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=0.5,minimum width=5cm, rounded corners=2pt, minimum height=2cm,inner ysep=1em, callout absolute pointer={(6.5,1.4)}] at (10,1.8) {\LARGE$\begin{cases}
	 				\abst{f}{E}  &\textrm{if}~\exists \abstfe.\ sat^+(\abst{f}{E}, \pex) \land sat^-(\abst{f}{E}, \nex)\\
	 				\bot &\textrm{otherwise}
	 			\end{cases}$};
	 	}
	 	\uncover<3->{
	 		\node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=0.5,minimum width=5cm, rounded corners=2pt, minimum height=2cm,inner ysep=1em, callout absolute pointer={(7,0.5)}] at (11,-.4) {\LARGE$\begin{cases}
	 			\mathtt{True},$ if $\forall a. \abst{\hat{f}}{}(a) \sqsubseteq \abst{f}{E}(a)\\
	 			\mathtt{False}, \langle a,c'\rangle$, if $\exists \langle a,c'\rangle$, such that $c' \in \gamma(\abst{\hat{f}}{}(a)) \setminus \gamma(\abst{f}{E}(a))
	 			\end{cases}$};
	 	}
	 	
	 	\uncover<4->{
	 		\node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=0.5,minimum width=5cm, rounded corners=2pt, minimum height=2cm,inner ysep=1em, callout absolute pointer={(7,-1.6)}] at (11,-2.4) {\LARGE$\begin{cases}
	 			\mathtt{False}, \langle a,c'\rangle$, if $\exists \langle a,c'\rangle $, such that $c' \in \gamma(\abst{f}{E}(a)) \setminus \gamma(\abst{\hat{f}}{L}(a))\\
	 			 \texttt{True}, \textrm{\ otherwise}. 
	 			\end{cases}$};
	 	}
	 }
\scalebox{0.73}{
	\centering
	\hspace{3cm}
\begin{algorithm2e}[H]
    \setcounter{algocf}{0}
	\caption {\textsc{SynthesizeTransformer}($f$) // $C, A, \sqcup, \gamma, \alpha, \beta, L$\label{Alg:main}}
	
	$\abst{f}{E} \leftarrow \lambda a: \bot$\\
	$isSound, isPrecise \gets False$\\
	$\pex, \nex \gets \func{InitializeExamples()}$ \label{Alg:main:sampling}
	
	\While{$\lnot \textit{isSound} \lor \lnot \textit{isPrecise}$} {      \label{Alg:main:outerwhile}
		%		$\abst{f}{curr} \gets \abst{f}{E}$\\
		 {
			%                        \twr{Why does $\func{Synthesize}$ take $\abst{f}{curr}$ and not $f$ as an argument?}
			\label{Alg:main:isconsistent}
			$\abst{f}{E} \gets \func{Synthesize}( \pex, \nex)$ \label{Alg:main:gentransformer}
		}
	
		\If{$*$} { \label{Alg:main::if-nondet}
			%\If{$\lnot \textit{isSound}$} 
			{ \label{Alg:main:sound}
				%              \twr{Why does $\func{CheckSoundness}$ set $\textit{isPrecise}$?} \\
				$\textit{isSound}, e \gets \func{CheckSoundness*}(\abst{f}{E}, f, \pex, \nex)$\\
				\If{$\lnot \textit{isSound}$}{
					{$\textit{isPrecise} \gets \bot$}\\
					$\pex \gets \pex \cup \{e\}$ \label{Alg:main:AdjustEPlus}
				}
			}
		}
		
		\Else {
			%\If{$\lnot \textit{isPrecise}$} 
			{ \label{Alg:main:precise}
				%               \twr{Why does $\func{CheckPrecision}$ set $\textit{isSound}$?} \\
				$\textit{isPrecise}, e \gets \func{CheckPrecision*}(\abst{f}{E}, \pex, \nex)$\\
				\If{$\lnot isPrecise$}{
					{$\textit{isSound} \gets \bot$}\\
					$\nex \gets \nex \cup \{e\}$ \label{Alg:main:AdjustEMinus}
				}
			}
		}
		
	}
	\Return { $\abst{f}{E}$ }
\end{algorithm2e}
}
\end{frame}



==> slides/prob_stmt.tex <==

\begin{frame}{Problem statement}
    \begin{center}
        \textcolor{blue}{Can we automatically \textit{synthesize} an abstract transformer for black-box operations?}
    \end{center}
    \pause

    \begin{block}{}
Given the 
        \begin{itemize}
            \item executable semantics $\llbracket f \rrbracket$ of a concrete transformer $f$, 
            \item description of an abstract domain ($A, \sqsubseteq, \sqcup$), and its relation to the concrete domain ($\alpha, \gamma, \beta$), and 
            \item a domain-specific language $L$, 
        \end{itemize}

        synthesize the \textbf{best} abstract transformer $\widehat{\abst{f}{}}$ of $f$ for $A$ in $L$. %that is in the set of most-precise, sound abstract transformers that are expressible in $L$.
    \end{block}
\end{frame}

\begin{frame}{The magic we need...}
    Given the following domain-specific language, we desire to get an abstract transformer for \textcolor{blue}{Math.abs} in the \textcolor{blue}{interval domain}:
    \textcolor{blue}{
	\begin{equation*}
	\label{Eq:LForIntervalDomain}
	\begin{footnotesize}
	\begin{array}{r@{\hspace{1.0ex}}c@{\hspace{1.0ex}}l}
	\small
	\textit{Transformer} & ::= & \lambda \texttt{a} . [E, E] \\
	E & ::= & \texttt{a.l}\ |\ \texttt{a.r}\ |\ 0\ |\ {-}E\ |\ {+}\infty\ |\ {-}\infty |\  E + E\ |\ E - E\ |\ E * E\ |\ \texttt{min}(E, E)\ |\ \texttt{max}(E, E)
	\end{array}
	\end{footnotesize}                
	\end{equation*}
    }%
	%
	\uncover<2->{
		\tikz[remember picture,overlay]{
			\node[rectangle callout,draw=red, fill=aliceblue,inner sep=2pt,align=center,aspect=2,scale=0.5,minimum width=5cm, rounded corners=2pt, minimum height=2cm,inner ysep=1em, callout absolute pointer={(5,1.15)}] at (9.5,2) {\LARGE \texttt{a.l}: Left limit \\[1em]  \LARGE \ \ \texttt{a.r}: Right limit};
		}
	}
	\pause
	\pause
	%
    We could emit one of the following abstract transformers:\\[2em]
	\begin{center}
	\fcolorbox{red}{mymauve!30}{
	$
	\mathtt{\abst{abs}{1}(a: \intv) : \intv = [max(max(0, a.l), -a.r), \ max(-a.l, a.r)]}
	$
	}\\[1em]
	\fcolorbox{red}{mymauve!30}{
	$
	\mathtt{abs^\sharp_2 (a: \intv) : \intv =[max(0, a.l)-min(0, a.r), \ max(-a.l, a.r)]}
	$%
}%
	\pause
	\end{center}
    The transformers must be sound and maximally-precise.
    \end{frame}

\begin{frame}{Challenges}
	\begin{enumerate}
        \item $\widehat{\abst{f}{}}$ may not be computable; it can be expressed as \[\abst{\widehat{f}}{} = \lambda a: \sqcup \{ \beta(f(c_i)) \ |\ c_i \in \gamma(a) \}\]%
            \vspace{-15pt} \pause%
        \item $\widehat{\abst{f}{}}$ may not be expressible in $L$
            \pause
        \item Precision defines a partial ordering on abstract transformers, so $\bestl$ may not be unique %\todo{give example from paper}
        \pause
            Example: \texttt{f(x) = 0},  $L = \{\lambda a.\ [0,k], \lambda a.\ [-k, 0]\ \mid k\in \mathbb{N} \wedge k\geq 1 \}$, $\abst{\widehat{\mathcal{S}}}{L} = \{ \lambda a. [0,1], \lambda a. [-1, 0]\}$
	\end{enumerate}
    \pause
    \begin{block}{\emph{best $L$-transformer}}
	    	An abstract transformer $\abst{f}{L} \in L$ is a \textbf{\emph{best $L$-transformer}} (denoted as $\bestl$) if $\abst{f}{L}$ is both sound and there does not exist any other transformer in $L$ that is more precise.
    \end{block}

\end{frame}

\begin{frame}{Problem statement (revised)}

    \begin{block}{}
Given the 
        \begin{itemize}
            \item executable semantics $\llbracket f \rrbracket$ of a concrete transformer $f$, 
            \item description of an abstract domain ($A, \sqsubseteq, \sqcup$), and its relation to the concrete domain ($\alpha, \gamma, \beta$), and 
            \item a domain-specific language $L$, 
        \end{itemize}

        synthesize \textbf{a best L-transformer} $\widehat{\abst{f}{L}}$ of $f$ for $A$ in $L$. %that is in the set of most-precise, sound abstract transformers that are expressible in $L$.
    \end{block}

    \only<2>{
        We build a tool, \tool\footnote{The Hindi word \includegraphics[scale=.32,trim={0 0.28cm 0 0},clip]{fig/amurth.pdf} means \textit{abstract}}, that solves the above problem.}
\end{frame}

    \begin{frame}[fragile]{Who cares?}

    \begin{itemize}
        \item even simple function, on simple abstract domains, may require non-trivial abstract transformers
        \item writing transformers manually is error-prone; we found multiple bugs in abstract transformers in the string analysis tool \safestr\footnote{\tiny R. Amadini, A. Jordan, G. Gange, F. Gauthier, P. Schachte, H. Søndergaard, P. J. Stuckey \& C. Zhang, ``Combining String Abstract Domains for JavaScript Analysis: An Evaluation'', in TACAS’17}
    \end{itemize}
        \begin{center}
        \pause
        \vspace{10pt}
        \tool can synthesize non-trivial transformers, with only black-box access to the concrete function, in reasonable time (600-1500 seconds).\\
        \pause
        \vspace{10pt}
        Now, let's dive into the workings of \tool.
        \end{center}
	
\end{frame}
	

